From Monge to Higgs: a survey of distance computations in noncommutative geometry

This is a review of explicit computations of Connes distance in noncommutative geometry, covering finite dimensional spectral triples, almost-commutative geometries, and spectral triples on the algebra of compact operators. Several applications to physics are covered, like the metric interpretation of the Higgs field, and the comparison of Connes distance with the minimal length that emerges in various models of quantum spacetime. Links with other areas of mathematics are studied, in particular the horizontal distance in sub-Riemannian geometry. The interpretation of Connes distance as a noncommutative version of the Monge-Kantorovich metric in optimal transport is also discussed.

==> commandes.tex <==
%%%%%%%%%%%%%% couleurs %%%%%%%%%%%%%%%%%%%%%%%
\definecolor{bleuvert}{rgb}{.1,.5,.4}
 %\definecolor{grispale}{rgb}{.8,.9,.9}
\definecolor{light-gray}{gray}{0.95}
\definecolor{gray}{gray}{0.75}
\definecolor{violet}{rgb}{0.4,0.,0.3}
\definecolor{jaune}{rgb}{0.8,0.6,0.1}
\definecolor{cvert}{rgb}{0.8,0.6,0.5}
\newcommand{\rosso}[1]{{\color{red} #1}}
\newcommand{\bleuvert}[1]{{\color{bleuvert} #1}} 
\newcommand{\cvert}[1]{{\color{cvert} #1}} 
\newcommand{\purple}[1]{{\color{purple} #1}} 
\newcommand{\violet}[1]{{\color{violet} #1}} 
\newcommand{\comm}[1]{{\bf\rosso{[#1]}}} 
\newcommand{\segna}[1]{\sout{#1}}
\newcommand{\bleu}[1]{{\color{bleu} #1}} 
%  \definecolor{couleur}{rgb}{.1,.5,.4}
%  \newcommand{\couleur}[1]{{\color{couleur} #1}} 
%%%%%%%%%%%%%% théorème %%%%%%%%%%%%%%%%%%%%%%%
\newtheorem{thm}{Theorem}[section]
\newtheorem{lem}[thm]{Lemma}
\newtheorem{prop}[thm]{Proposition}
\newtheorem{cor}[thm]{Corollary}
\newtheorem{defi}[thm]{Definition}
\newtheorem{rem}[thm]{Remark}
\newenvironment{preuve}{{\emph{Proof.}}}{\hfill$\blacksquare$}

% \newcommand{\A}{\mathcal{A}}
% \newcommand{\B}{\mathcal{B}}
% \newcommand{\HH}{\mathcal{H}}
% \newcommand{\N}{\mathbb{N}}
% \newcommand{\Z}{\mathbb{Z}}
% \newcommand{\R}{\mathbb{R}}
% \newcommand{\C}{\mathbb{C}}
% \newcommand{\P}{\mathbb{P}}
% \newcommand{\S}{\mathbb{S}}
%%%%%%%%%%%%%% norme %%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\norm}[1]{\left\lVert#1\right\rVert}
\newcommand{\abs}[1]{\lvert#1\rvert}
\newcommand{\scal}[1]{\langle#1,#1\rangle}
\newcommand{\scl}[2]{\langle#1,#2\rangle}
\newcommand{\suup}[1]{ \underset{#1}{\sup} }
\newcommand{\suum}[2]{\overset{#2}{\underset{#1}{\Sigma}}}
\newcommand{\grad}[1]{\text{grad}\,#1}
\newcommand{\tra}[1]{\text{Tr}\; #1}
\newcommand{\ket}[1]{\lvert#1\rangle}
\newcommand{\bra}[1]{\langle#1\lvert}
\newcommand{\ST}{C\hspace{-1pt}S}
%\newcommand{\tr}[1]{\text{Tr}(#1)}
%\newcommand{\binom}[2]{\left( \begin{array}{c} #1 #2 \end{array}\right)}
\def\begf{\begin{frame}}
\def\enf{\end{frame}}
\def\opm{\only<+->}
\def\begz{\begin{itemize}}
\def\ipm{\item<+->}
\def\endz{\end{itemize}}
\def\upm{\uncover<+->}
\def\odanois{\o}
\def\lp{\left(} 
\def\rp{\right)} 
\def\dm{\lp\begin{array}}	
\def\fm{\end{array}\rp}
\def\begf{\begin{frame}}
\def\enf{\end{frame}}
\def\opm{\only<+->}
\def\begz{\begin{itemize}}
\def\ipm{\item<+->}
\def\endz{\end{itemize}}
\def\upm{\uncover<+->}
\def\odanois{\o}
\def\lp{\left(} 
\def\rp{\right)} 
\def\dm{\lp\begin{array}}	
\def\fm{\end{array}\rp}
\def\m2{M_2 \lp \cc \rp}
\def\m3{M_3 \lp \cc \rp}	
\def\mn{M_n \lp \cc \rp}	
\def\re{\text{Re}}			
\def\im{\text{Im}}
\def\ot{\otimes}

\def\ds{\partial\!\!\!\slash}
\def\sh{\text{sh}}
\def\ch{\text{ch}}
		
\def\kk{{\mathbb{K}}}	
\def\cc{{\mathbb{C}}}
\def\C{{\mathbb{C}}}	
\def\rr{{\mathbb{R}}}
\def\R{{\mathbb{R}}}
\def\nn{{\mathbb{N}}}
\def\N{{\mathbb{N}}}
\def\zz{{\mathbb{Z}}} 		
\def\ii{{\mathbb{I}}}
\def\I{{\mathbb{I}}}
\def\hhh{{\mathbb H}}
\newcommand{\id}{\mathbbm{1}}

\def\ee{{\cal E}}
\def\E{{\cal E}}
\def\F{{\cal F}}	
\def\mm{{\mathcal M}}	
\def\M{{\mathcal M}}		
\def\aa{{\mathcal A}}
\def\ak{{\mathfrak A}}
\def\A{{\mathcal A}}			
\def\bb{{\mathcal B}}			
\def\ll{{\mathcal L}}
\def\dd{{\mathcal D}}	
\def\hh{{\mathcal H}}
\def\jj{{\mathcal J}}
\def\oo{{\mathcal O}}
\def\pp{{\mathcal P}}
\def\ccc{{\mathcal C}}
\def\jj{{\mathcal J}}
\def\gg{{\mathcal G}}
\def\X{{\mathcal X}}
\def\xx{{\bf x}}
\def\yy{{\bf y}}
\def\ss{{\mathcal S}}
\def\iii{{\mathcal I}}
\def\K{{\mathcal K}}
\def\BH{{\mathcal B}({\mathcal H})}
\def\zzz{{\bf z}}
\def\bda{{{\mathcal B}_D(\A)}}
\def\bl{{{\mathcal B}_{\text{Lip}}}}
\def\cinf{C^{\infty}\lp\mm\rp}
\def\coi{C^{\infty}_0\lp\mm\rp}
\def \difm{\text{Diff}({\mathcal{M}})}
\def\cm{C^{\infty}(\mm)}
\def\nabc{\nabla_{\!\!\dot{c}_*}}
\def\nabm{\nabla_{\!\!\mu}}
\def\As{\A_{\star}}
\def\lda{\text{Lip}_D(\A)}

\def\xox{{\xi}_x}
\def\yox{{\xi}_y}
\def\xoz{{\zeta}_x}
\def\yoz{{\zeta}_y}
\def\ox{\omega_{\xi}}
\def\oz{\omega_{\zeta}}
\def\op{\omega_{\psi}}
\def\opp{\omega_{\tilde\psi}}
\def\opu{\omega_{\psi,1}}
\def\oppd{\omega_{\psi',2}}

%******* vecteurs et etats **************
\def\ot{\otimes}
\def\pof{\psi\otimes\xi}
\def\fop{\xi\otimes\psi}

\def\xox{{\xi}_x}
\def\yox{{\xi}_y}
\def\xoz{{\zeta}_x}
\def\yoz{{\zeta}_y}

\def\omx{\omega_x}
\def\omy{\omega_y}

\def\ox{\omega_{\xi}}
\def\oz{\omega_{\zeta}}
\def\xo0{\omega^0_x}
\def\yo0{\omega^0_y}
\def\tox{\tilde{\omega_{\xi}}}
\def\toz{\tilde{\omega_{\zeta}}}
\def\oe{\omega_{E}}
\def\oi{\omega_{I}}
\def\oei{\omega_{E}\ot\omega_{I}}
\def\oeip{\omega_{E}\ot\omega_{I}'}
\def\oepi{\omega_{E}'\ot\omega_I }
\def\oepip{ {\omega_E}' \ot {\omega_I}'}
\def\xoi{\omega_x\ot\omega_i}
\def\xoip{\omega_x\ot\omega_{i}'}
\def\yoi{\omega_y\ot\omega_i}
\def\yoip{\omega_y\ot\omega_{i}'}

\def\ou{{\omega_{1}}}
\def\od{{\omega_{2}}}
\def\odu{\omega_{21}}
\def\oud{{\omega_{12}}}
\def\opud{{{\omega'}_{12}}}
\def\opdu{{{\omega'}_{21}}}
\def\ou{{\omega_{1}}}
\def\ouu{{\omega_{11}}}
\def\odd{{\omega_{22}}}
\def\oc{{\omega_{c}}}
\def\oeu{\omega_E \ot \ou}
\def\oed{\omega_E \ot \od}
\def\oeo{\omega_E \ot \omega}

\def\omm{\omega_m}
\def\omn{\omega_n}
\def\akom{\alpha_\kappa\omega_m}
\def\akton{\alpha_{\tilde\kappa}\omega_n}

\def\roe{\rho_E}
\def\rope{\rho'_E}
\def\roi{\rho_I}
\def\ropi{\rho'_I}
\def\roei{(\rho_E,\rho_I)}

\def\oxe{\omega_{k_e}}
\def\oze{\omega_{{k'}_e}}
\def\oue{\omega_{1}\circ\alpha_e}
\def\ode{\omega_{2}\circ\alpha_e}
%\def\o0{\omega_0}
\def\rx{\rho_\xi}
\def\rz{\rho_\zeta}
\def\sx{s_\xi}
\def\sz{s_\zeta}

\def\xk{x_{k}}
\def\yk{y_{k}}
\def\rk{\rho_k}
\def\rkp{\rho_{k'}}
\def\ux{{u_k}}
\def\uz{{u_{k'}}}
\def\xkp{x_{{k'}}}
\def\ykp{y_{{k'}}}
\def\xo0{x_\omega^0}
\def\yo0{y_\omega^0}
\def\tox{\tilde{\omega_{k}}}
\def\toz{\tilde{\omega_{{k'}}}}
\def\nx{{n_k}}
\def\nz{{n_{k'}}}

\def\ale{\alpha_e}
\def\aea{\alpha_e(\aa)}
\def\fu{\alpha_u}
\def\fue{\alpha_{u^*}}
\def\tu{\tau_1}
\def\td{\tau_2}
\def\futu{\fu(\tu)}
\def\futd{\fu(\td)}
\def\fuetu{\fue(\tu)}
\def\fuetd{\fue(\td)}
\def\tue{\tu\circ\ae}
\def\tde{\td\circ\ae}

\def\te{\tau_E}
\def\ti{\tau_I}
\def\tei{\tau_E\ot\tau_I}
\def\po{\pi_\omega}
\def\pto{\tilde{\pi}_\omega}

\def\gtl{g_{\tilde\lambda}}
\def\fll{f_{\lambda}}

\def\auta{\text{Aut}(\aa)}
\def\ina{\text{In(\aa)}}
\def\outa{\text{Out}(\aa)}\def\auta{\text{Aut}(\aa)}
\def\inmn{\text{In}(\mn)}
\def\outmn{\text{Out}(\mn)}

\def\cl{\text{Cl}}
\def\ccl{\cc\text{l}}

\def\pa{{\mathcal P}(\aa)}
\def\sa{{\mathcal S}(\aa)}
\def\qq{{\mathcal Q}}


\def\ssquare{{\text{\tiny $\blacksquare$}}}
%\def\tt{{\mathbb T}_\theta}
\def\aat{\aa_\theta}
\def\at{{A_\theta}}
\def\hht{{\hh_\theta}}
\def\dt{{D_\theta}}
\def\nabc{\nabla_{\!\!\dot{c}_*}}
\def\nabm{\nabla_{\!\!\mu}}
\def\iii{{\mathcal I}}
\def\xm{x^\mu}
\def\xn{x^\nu}
\def\xr{x^\rho}
\def\xl{x^\lambda}
\def\fm{\Phi(x^\mu)}
\def\fn{\Phi(x^\nu)}
\def\fr{\Phi(x^\rho)}
\def\fl{\Phi(x^\lambda)}
\def\dm{\partial_\mu}
\def\dn{\partial_\nu}
\def\X{{\mathcal X}}
\def\NN{{\mathcal N}}
\def\dmm{\left(\begin{array}}
\def\fmm{\end{array}\right)}

\newcommand{\tdx}{\tilde{\mathbf{x}}}


\newcommand{\HH}{\mathcal{H}}
\newcommand{\de}{\mathrm{d}}
\newcommand{\abso}[1]{|#1|}
\newcommand{\dc}{d_D}
\newcommand{\inner}[1]{\left<#1\right>}
\newcommand{\ma}[2]{\left(\!\rule{0pt}{#1}\smash[b]{\smash[t]{\begin{array}{cc}#2\end{array}}}\!\right)}

		
